Beyond Highway Dimension: Small Distance Labels Using Tree Skeletons

The goal of a hub-based distance labeling scheme for a network G = (V, E) is to assign a small subset S(u) $\subseteq$ V to each node u $\in$ V, in such a way that for any pair of nodes u, v, the intersection of hub sets S(u) $\cap$ S(v) contains a node on the shortest uv-path. The existence of small hub sets, and consequently efficient shortest path processing algorithms, for road networks is an empirical observation. A theoretical explanation for this phenomenon was proposed by Abraham et al. (SODA 2010) through a network parameter they called highway dimension, which captures the size of a hitting set for a collection of shortest paths of length at least r intersecting a given ball of radius 2r. In this work, we revisit this explanation, introducing a more tractable (and directly comparable) parameter based solely on the structure of shortest-path spanning trees, which we call skeleton dimension. We show that skeleton dimension admits an intuitive definition for both directed and undirected graphs, provides a way of computing labels more efficiently than by using highway dimension, and leads to comparable or stronger theoretical bounds on hub set size.

==> Makefile <==
# Mettre les .tex et les .bib dans ce répertoire, les figures dans figs/

DOCS=$(wildcard *.tex)
DOCS_BASE=$(subst .tex,,$(DOCS))
DOC=$(word 1, $(DOCS_BASE))

FIGS=$(wildcard figs/*.pdf)

BIBS=$(wildcard *.bib)
BIB=$(word 1, $(BIBS))


dft: $(DOC).pdf

one: $(DOC).one

echo:
	echo "DOC:$(DOC) BIB:$(BIB) FIGS:$(FIGS)"


%.one: %.tex
	pdflatex $<
	make menage


%.pdf: %.tex $(FIGS) $(BIBS)
	pdflatex $< ;\
	if grep bibdata $*.aux > /dev/null ; then \
		echo bibtex --------------------------------- ;\
		bibtex $* ;\
		pdflatex $< ;\
		(bibtex $* | grep undefined) || echo -n ;\
	fi ;\
	(pdflatex $< | grep defined) || echo -n
	make menage


menage:
	rm -f *.log *.bbl *.blg *.aux *.snm *.out *.nav *.toc || echo menage


clean: menage
	rm -f *~







